LX-mixers for QAOA: Optimal mixers restricted to subspaces and the stabilizer formalism

We present a novel formalism to both understand and construct mixers that preserve a given subspace. The method connects and utilizes the stabilizer formalism that is used in error correcting codes. This can be useful in the setting when the quantum approximate optimization algorithm (QAOA), a popular meta-heuristic for solving combinatorial optimization problems, is applied in the setting where the constraints of the problem lead to a feasible subspace that is large but easy to specify. The proposed method gives a systematic way to construct mixers that are resource efficient in the number of controlled not gates and can be understood as a generalization of the well-known X and XY mixers and a relaxation of the Grover mixer: Given a basis of any subspace, a resource efficient mixer can be constructed that preserves the subspace. The numerical examples provided show a dramatic reduction of CX gates when compared to previous results. We call our approach logical X-Mixer or logical X QAOA ($\textbf{LX-QAOA}$), since it can be understood as dividing the subspace into code spaces of stabilizers S and consecutively applying logical rotational X gates associated with these code spaces. Overall, we hope that this new perspective can lead to further insight into the development of quantum algorithms.

==> statistics_cnots_n4_4.tex <==
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{goldenrod1911910}{RGB}{191,191,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{yellow}{RGB}{255,255,0}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle |B|\)},
xmin=2, xmax=16,
xtick style={color=black},
y grid style={darkgray176},
ylabel={#CNOTS},
ymin=-23.2, ymax=487.2,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.35]
(axis cs:2,4.05205392067787)
--(axis cs:2,0.787946079322132)
--(axis cs:3,9.02085538350015)
--(axis cs:4,9.9217548361769)
--(axis cs:5,15.0941514062269)
--(axis cs:6,20.2298643777933)
--(axis cs:7,20.5340451116064)
--(axis cs:8,24.2608056006245)
--(axis cs:9,27.0152310422805)
--(axis cs:10,33.0217185178383)
--(axis cs:11,29.3997489572711)
--(axis cs:12,23.0684555186986)
--(axis cs:13,15.8077037206369)
--(axis cs:14,8.39579335435692)
--(axis cs:15,8)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:15,8)
--(axis cs:14,12.9642066456431)
--(axis cs:13,20.9922962793631)
--(axis cs:12,36.7315444813014)
--(axis cs:11,48.520251042729)
--(axis cs:10,47.2182814821617)
--(axis cs:9,42.7047689577195)
--(axis cs:8,38.6591943993755)
--(axis cs:7,44.3859548883936)
--(axis cs:6,31.2901356222067)
--(axis cs:5,23.7858485937731)
--(axis cs:4,16.7582451638231)
--(axis cs:3,15.0991446164998)
--(axis cs:2,4.05205392067787)
--cycle;
\addlegendimage{area legend, draw=green, fill=green, opacity=0.35}
\addlegendentry{$1\sigma$}

\path [draw=black, fill=black, opacity=0.15]
(axis cs:2,6)
--(axis cs:2,0)
--(axis cs:3,6)
--(axis cs:4,2)
--(axis cs:5,12)
--(axis cs:6,12)
--(axis cs:7,10)
--(axis cs:8,10)
--(axis cs:9,22)
--(axis cs:10,14)
--(axis cs:11,20)
--(axis cs:12,8)
--(axis cs:13,14)
--(axis cs:14,8)
--(axis cs:15,8)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:15,8)
--(axis cs:14,16)
--(axis cs:13,22)
--(axis cs:12,40)
--(axis cs:11,64)
--(axis cs:10,52)
--(axis cs:9,52)
--(axis cs:8,40)
--(axis cs:7,52)
--(axis cs:6,36)
--(axis cs:5,34)
--(axis cs:4,22)
--(axis cs:3,16)
--(axis cs:2,6)
--cycle;

\path [draw=blue, fill=blue, opacity=0.35]
(axis cs:2,40.2082156827115)
--(axis cs:2,27.1517843172885)
--(axis cs:3,52.5301638287575)
--(axis cs:4,66.7151920463258)
--(axis cs:5,62.5475419626693)
--(axis cs:6,58.7893250517617)
--(axis cs:7,49.6358958450058)
--(axis cs:8,37.7718899362986)
--(axis cs:9,37.340886594508)
--(axis cs:10,39.4980968481525)
--(axis cs:11,29.3997489572711)
--(axis cs:12,23.0684555186986)
--(axis cs:13,15.8077037206369)
--(axis cs:14,8.39579335435692)
--(axis cs:15,8)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:15,8)
--(axis cs:14,12.9642066456431)
--(axis cs:13,20.9922962793631)
--(axis cs:12,36.7315444813014)
--(axis cs:11,48.520251042729)
--(axis cs:10,53.5819031518475)
--(axis cs:9,48.619113405492)
--(axis cs:8,53.9081100637014)
--(axis cs:7,64.8441041549942)
--(axis cs:6,96.5706749482384)
--(axis cs:5,113.932458037331)
--(axis cs:4,96.0048079536742)
--(axis cs:3,67.7898361712425)
--(axis cs:2,40.2082156827115)
--cycle;
\addlegendimage{area legend, draw=blue, fill=blue, opacity=0.35}
\addlegendentry{$1\sigma$}

\path [draw=black, fill=black, opacity=0.15]
(axis cs:2,48)
--(axis cs:2,24)
--(axis cs:3,48)
--(axis cs:4,24)
--(axis cs:5,40)
--(axis cs:6,32)
--(axis cs:7,32)
--(axis cs:8,32)
--(axis cs:9,32)
--(axis cs:10,14)
--(axis cs:11,20)
--(axis cs:12,8)
--(axis cs:13,14)
--(axis cs:14,8)
--(axis cs:15,8)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:16,0)
--(axis cs:15,8)
--(axis cs:14,16)
--(axis cs:13,22)
--(axis cs:12,40)
--(axis cs:11,64)
--(axis cs:10,60)
--(axis cs:9,56)
--(axis cs:8,72)
--(axis cs:7,72)
--(axis cs:6,128)
--(axis cs:5,136)
--(axis cs:4,104)
--(axis cs:3,72)
--(axis cs:2,48)
--cycle;

\path [draw=red, fill=red, opacity=0.35]
(axis cs:2,40.2082156827115)
--(axis cs:2,27.1517843172885)
--(axis cs:3,56.4602222252706)
--(axis cs:4,87.701938411554)
--(axis cs:5,116.241342357463)
--(axis cs:6,144.163060429174)
--(axis cs:7,177.801587401581)
--(axis cs:8,203.977794898144)
--(axis cs:9,232.243301301535)
--(axis cs:10,258.168993144399)
--(axis cs:11,289.044484868667)
--(axis cs:12,318.348324543876)
--(axis cs:13,343.249405469573)
--(axis cs:14,371.945415939958)
--(axis cs:15,397.191445061784)
--(axis cs:16,426.195523135907)
--(axis cs:16,453.004476864093)
--(axis cs:16,453.004476864093)
--(axis cs:15,429.368554938216)
--(axis cs:14,400.374584060042)
--(axis cs:13,374.030594530427)
--(axis cs:12,348.371675456124)
--(axis cs:11,324.715515131333)
--(axis cs:10,293.031006855601)
--(axis cs:9,265.196698698465)
--(axis cs:8,232.822205101856)
--(axis cs:7,202.998412598419)
--(axis cs:6,173.436939570826)
--(axis cs:5,140.078657642537)
--(axis cs:4,111.018061588446)
--(axis cs:3,72.6597777747294)
--(axis cs:2,40.2082156827115)
--cycle;
\addlegendimage{area legend, draw=red, fill=red, opacity=0.35}
\addlegendentry{$1\sigma$}

\path [draw=black, fill=black, opacity=0.15]
(axis cs:2,48)
--(axis cs:2,24)
--(axis cs:3,48)
--(axis cs:4,80)
--(axis cs:5,104)
--(axis cs:6,128)
--(axis cs:7,160)
--(axis cs:8,176)
--(axis cs:9,200)
--(axis cs:10,232)
--(axis cs:11,264)
--(axis cs:12,304)
--(axis cs:13,328)
--(axis cs:14,360)
--(axis cs:15,376)
--(axis cs:16,408)
--(axis cs:16,464)
--(axis cs:16,464)
--(axis cs:15,448)
--(axis cs:14,416)
--(axis cs:13,400)
--(axis cs:12,368)
--(axis cs:11,344)
--(axis cs:10,320)
--(axis cs:9,296)
--(axis cs:8,256)
--(axis cs:7,224)
--(axis cs:6,192)
--(axis cs:5,160)
--(axis cs:4,136)
--(axis cs:3,80)
--(axis cs:2,48)
--cycle;

\path [draw=yellow, fill=yellow, opacity=0.35]
(axis cs:2,4.05205392067787)
--(axis cs:2,0.787946079322132)
--(axis cs:3,10.2909940348785)
--(axis cs:4,14.2395850800994)
--(axis cs:5,21.415221987096)
--(axis cs:6,39.0858116886745)
--(axis cs:7,65.0651511055787)
--(axis cs:8,84.0897423609772)
--(axis cs:9,102.874376029591)
--(axis cs:10,126.916442243858)
--(axis cs:11,166.071072253301)
--(axis cs:12,223.370960191056)
--(axis cs:13,295.055707728852)
--(axis cs:14,346.838629215269)
--(axis cs:15,397.191445061784)
--(axis cs:16,426.195523135907)
--(axis cs:16,453.004476864093)
--(axis cs:16,453.004476864093)
--(axis cs:15,429.368554938216)
--(axis cs:14,392.361370784731)
--(axis cs:13,344.544292271148)
--(axis cs:12,282.629039808944)
--(axis cs:11,228.088927746699)
--(axis cs:10,169.643557756142)
--(axis cs:9,133.605623970409)
--(axis cs:8,106.990257639023)
--(axis cs:7,89.0548488944213)
--(axis cs:6,65.2341883113255)
--(axis cs:5,37.744778012904)
--(axis cs:4,23.8804149199006)
--(axis cs:3,16.8290059651215)
--(axis cs:2,4.05205392067787)
--cycle;
\addlegendimage{area legend, draw=yellow, fill=yellow, opacity=0.35}
\addlegendentry{$1\sigma$}

\path [draw=black, fill=black, opacity=0.15]
(axis cs:2,6)
--(axis cs:2,0)
--(axis cs:3,6)
--(axis cs:4,12)
--(axis cs:5,14)
--(axis cs:6,24)
--(axis cs:7,50)
--(axis cs:8,60)
--(axis cs:9,88)
--(axis cs:10,104)
--(axis cs:11,120)
--(axis cs:12,176)
--(axis cs:13,260)
--(axis cs:14,320)
--(axis cs:15,376)
--(axis cs:16,408)
--(axis cs:16,464)
--(axis cs:16,464)
--(axis cs:15,448)
--(axis cs:14,416)
--(axis cs:13,384)
--(axis cs:12,332)
--(axis cs:11,268)
--(axis cs:10,208)
--(axis cs:9,160)
--(axis cs:8,124)
--(axis cs:7,96)
--(axis cs:6,96)
--(axis cs:5,50)
--(axis cs:4,34)
--(axis cs:3,20)
--(axis cs:2,6)
--cycle;

\addplot [semithick, green01270, mark=x, mark size=3, mark options={solid}]
table {%
2 2.42
3 12.06
4 13.34
5 19.44
6 25.76
7 32.46
8 31.46
9 34.86
10 40.12
11 38.96
12 29.9
13 18.4
14 10.68
15 8
16 0
};
\addlegendentry{mean , optimal reduced}
\addplot [semithick, black, dotted, mark=x, mark size=3, mark options={solid}, forget plot]
table {%
2 0
3 6
4 2
5 12
6 12
7 10
8 10
9 22
10 14
11 20
12 8
13 14
14 8
15 8
16 0
};
\addplot [semithick, black, dotted, mark=x, mark size=3, mark options={solid}]
table {%
2 6
3 16
4 22
5 34
6 36
7 52
8 40
9 52
10 52
11 64
12 40
13 22
14 16
15 8
16 0
};
\addlegendentry{min/max , optimal reduced}
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
2 33.68
3 60.16
4 81.36
5 88.24
6 77.68
7 57.24
8 45.84
9 42.98
10 46.54
11 38.96
12 29.9
13 18.4
14 10.68
15 8
16 0
};
\addlegendentry{mean , optimal}
\addplot [semithick, black, dotted, mark=*, mark size=3, mark options={solid}, forget plot]
table {%
2 24
3 48
4 24
5 40
6 32
7 32
8 32
9 32
10 14
11 20
12 8
13 14
14 8
15 8
16 0
};
\addplot [semithick, black, dotted, mark=*, mark size=3, mark options={solid}]
table {%
2 48
3 72
4 104
5 136
6 128
7 72
8 72
9 56
10 60
11 64
12 40
13 22
14 16
15 8
16 0
};
\addlegendentry{min/max , optimal}
\addplot [semithick, red, mark=+, mark size=3, mark options={solid}]
table {%
2 33.68
3 64.56
4 99.36
5 128.16
6 158.8
7 190.4
8 218.4
9 248.72
10 275.6
11 306.88
12 333.36
13 358.64
14 386.16
15 413.28
16 439.6
};
\addlegendentry{mean , $T_{\Delta}$}
\addplot [semithick, black, dotted, mark=+, mark size=3, mark options={solid}, forget plot]
table {%
2 24
3 48
4 80
5 104
6 128
7 160
8 176
9 200
10 232
11 264
12 304
13 328
14 360
15 376
16 408
};
\addplot [semithick, black, dotted, mark=+, mark size=3, mark options={solid}]
table {%
2 48
3 80
4 136
5 160
6 192
7 224
8 256
9 296
10 320
11 344
12 368
13 400
14 416
15 448
16 464
};
\addlegendentry{min/max , $T_{\Delta}$}
\addplot [semithick, goldenrod1911910, mark=Mercedes star flipped*, mark size=3, mark options={solid}]
table {%
2 2.42
3 13.56
4 19.06
5 29.58
6 52.16
7 77.06
8 95.54
9 118.24
10 148.28
11 197.08
12 253
13 319.8
14 369.6
15 413.28
16 439.6
};
\addlegendentry{mean , $T_{\Delta}$, reduced}
\addplot [semithick, black, dotted, mark=Mercedes star flipped*, mark size=3, mark options={solid}, forget plot]
table {%
2 0
3 6
4 12
5 14
6 24
7 50
8 60
9 88
10 104
11 120
12 176
13 260
14 320
15 376
16 408
};
\addplot [semithick, black, dotted, mark=Mercedes star flipped*, mark size=3, mark options={solid}]
table {%
2 6
3 20
4 34
5 50
6 96
7 96
8 124
9 160
10 208
11 268
12 332
13 384
14 416
15 448
16 464
};
\addlegendentry{min/max , $T_{\Delta}$, reduced}
\end{axis}

\end{tikzpicture}

